Emergency Control of Transmission Voltages by Coordinating DERs From Multiple Substations

Voltage stability can be endangered in transmission networks that operate under high strain and exhibit a large separation between generators and loads. During emergencies associated to voltage instability, one promising supporting countermeasure is to control large populations of Distributed Energy Resources (DERs) connected to medium- and low-voltage networks, so that they locally reduce the net load by modifying their power generation or consumption. However, it is challenging to achieve this control while anticipating interactions with legacy voltage regulators, coordinating efforts across substations, and exchanging small amounts of information with DERs. In this paper, we propose a control scheme that coordinates DER aggregations with the load tap changers of substation transformers, asks them to contribute power depending on the substation they are connected to, and relies on lightweight communication. Our simulations show that the proposed control can successfully coordinate DERs and load tap changers to enhance long-term voltage stability.

==> figures/central_expanded.tex <==
\def\myA{0.02}
\def\myB{0.45}
\def\myC{0.16}
\def\myD{0.59}
\def\myfigwidth{12}
\def\myfigheight{12}
\begin{tikzpicture}
    \coordinate (origin) at (0, 0); 

    \begin{pgfonlayer}{map}
        \path[use as bounding box, clip] 
        (\myC*\myfigwidth, \myA*\myfigheight) rectangle (\myD*\myfigwidth, \myB*\myfigheight);
        \node (diagram) [anchor=south west,
                         inner sep=0pt]
           at (origin) {%
              \begin{tikzpicture}
                  \path[draw] (0, 0) rectangle ++(\myfigwidth, \myfigheight);
              \end{tikzpicture}
           };
    \end{pgfonlayer}

    \begin{pgfonlayer}{lines}
        \coordinate (origin) at (0, 0);
        \path[use as bounding box, clip] 
        % \draw 
        (\myC*\myfigwidth, \myA*\myfigheight) rectangle (\myD*\myfigwidth, \myB*\myfigheight);
    \end{pgfonlayer}

    \begin{pgfonlayer}{main}
        \coordinate (origin) at (0, 0);
        \path[use as bounding box, clip] 
        % \draw 
        (\myC*\myfigwidth, \myA*\myfigheight) rectangle (\myD*\myfigwidth, \myB*\myfigheight);

        % The following is based on https://tex.stackexchange.com/a/238352/75594
        \begin{scope}[
            x={(diagram.south east)},
            y={(diagram.north west)},
        ]

            \newcommand\xmin{0}
            \newcommand\xmax{0.99}
            \newcommand\ymin{0.0}
            \newcommand\ymax{0.835}

            % Draw legend
            \tikzset{nordic line/.style={400 kV lines}}

            % \drawregions
            % \drawlegend
            % \drawdata

            \tikzset{
                nordic bus/.style n args={4}{
                    power bus={#1}{#2}{#3}
                }
            }
            \tikzset{
                nordic bus/.style n args={4}{
                    transit,
                    region,
                    rounded rectangle,
                    inner sep=1.5pt,
                    node contents={
                        \ifthenelse{\equal{#1}{4061}}{\phantom{#1}}{%
                            \ifthenelse{\equal{#1}{4062}}{\phantom{#1}}{%
                                \ifthenelse{\equal{#1}{4063}}{\phantom{#1}}{%
                                    \ifthenelse{\equal{#1}{2031}}{\phantom{#1}}{%
                                        \ifthenelse{\equal{#1}{2032}}{\phantom{#1}}{%
                                            \ifthenelse{\equal{#1}{4031}}{\phantom{#1}}{%
                                                #1%
                                            }%
                                        }%
                                    }%
                                }%
                            }%
                        }%
                        % #1
                    },
                    font=\footnotesize,
                    #1,
                    name=#1
                    % simple bus={#1}{#2}{#3}{#4}
                }
            }
            \drawnordic[...]%[none]
        \end{scope}
    \end{pgfonlayer}

\end{tikzpicture}


==> tikzlibraryspyall.code.tex <==
% Spy all styles

\tikzset{
  spy all using outlines/.style={
    spy picture={
      every spy all on node/.style={very thin,draw},
      every spy all in node/.style={thick,draw},
      #1
    }
  },
  spy all using overlays/.style={
    spy picture={
      every spy all on node/.style={fill,fill opacity=0.2,text opacity=1},
      every spy all in node/.style={fill,fill opacity=0.2,text opacity=1},
      #1
    }
  },
  connect spies/.style={
    spy connection path={\draw[thin] (tikzspyonnode) -- (tikzspyinnode);}
  }
}

%\newbox\tikz@lib@spybox

\let\tikz@lib@spyall@collection=\pgfutil@empty%

\tikzset{spy picture/.style={
    size/.style={minimum size=##1},
    height/.style={minimum height=##1},
    width/.style={minimum width=##1},
    execute at begin picture={%
      \let\tikz@lib@spyall@save=\tikz@lib@spyall@collection%
      \let\spyall=\tikz@lib@spyall@parse%
      \tikz@insert@spy@layer
      \pgfonlayer{spy}%
    },
    execute at end picture={%
      \endpgfonlayer
      {%
        \tikz@lib@spyall@collection%
      }%
      \global\let\tikz@lib@spyall@collection=\tikz@lib@spyall@save%
    },%
    tikz@lib@spyall@style/.style={#1},
    tikz@lib@reset@gs
  },
  lens/.store in=\tikz@lib@spy@lens,
  lens=,
  magnification/.style={lens={scale=#1}},
  spy connection path/.store in=\tikz@lib@spy@path,
  spy connection path=
}

\tikzset{
  tikz@lib@reset@gs/.style={black,thin,solid,opaque,line cap=butt,line join=miter}
}

\def\tikz@lib@spyall@parse{%
  \pgfutil@ifnextchar[{\tikz@lib@spyall@parse@opt}{\tikz@lib@spyall@parse@opt[]}%]
}
\def\tikz@lib@spyall@parse@opt[#1]{
  \pgfutil@ifnextchar x{\tikz@lib@spyall@parse@opta[#1]}{\tikz@lib@spyall@parse@opta[#1]}%]
}
\def\tikz@lib@spyall@parse@opta[#1]on#2in node#3;{%
  \pgfutil@g@addto@macro\tikz@lib@spyall@collection{\tikz@lib@spyall@do{#1}{#2}{#3}}%
}

\def\tikz@lib@spyall@do#1#2#3{%
  \scope[tikz@lib@spyall@style,#1]
    \node [alias=tikzspyonnode,inner sep=0pt,outer sep=0pt,every spy all on node/.try,
    /utils/exec={
      {%
        \let\tikz@transform=\relax
        \pgftransformreset%
        \expandafter\tikzset\expandafter{\tikz@lib@spy@lens}
        \pgftransforminvert%
        \pgfgettransformentries\a\b\c\d\e\f%
        \global\let\pgf@lib@svg@a=\a%
        \global\let\pgf@lib@svg@b=\b%
        \global\let\pgf@lib@svg@c=\c%
        \global\let\pgf@lib@svg@d=\d%
      }%
      \tikz@addtransform{%
        \tikz@scan@one@point\pgftransformshift#2%
        \pgftransformcm{\pgf@lib@svg@a}{\pgf@lib@svg@b}{\pgf@lib@svg@c}{\pgf@lib@svg@d}{\pgfpointorigin}%
      }
    }]{};
    \node [alias=tikzspyinnode,inner sep=0pt,outer sep=0pt,at={#2},every spy all in node/.try,
    path picture={\node[anchor=center,tikz@lib@reset@gs]{\nullfont%
        \pgfpicture\relax\pgfsetbaseline{default}\pgfsettrimleft{default}\pgfsettrimright{default}%
        \pgftransformreset%
        \let\tikz@transform=\relax%
        \expandafter\tikzset\expandafter{\tikz@lib@spy@lens}%
        \pgflowlevelsynccm%
        \tikz@scan@one@point\tikz@lib@spyall@shift#2%
        \pgflowlevelsynccm%
        \pgf@dosavedlayers
        \endpgfpicture};}]#3{};
    \tikz@lib@spy@path
  \endscope
}

\def\tikz@lib@spyall@shift#1{%
  \pgf@process{#1}%
  \pgf@x=-\pgf@x%
  \pgf@y=-\pgf@y%
  \pgftransformshift{}%
}

\pgfdeclarelayer{spy}


\def\tikz@insert@spy@layer{%
    \expandafter\tikz@insert@spy@@layer\pgf@layerlist\relax
}
\def\tikz@insert@spy@@layer#1main#2\relax{%
    \def\pgf@layerlist{#1spy#2,main}%
}


\def\pgf@dosavedlayers{%
  \expandafter\pgf@dosavedlayer\pgf@layerlist,,\relax%
}
\def\pgf@dosavedlayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
    \copy\pgf@layerbox@main
  \else%
    \expandafter\copy\csname pgf@layerboxsaved@#1\endcsname
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dosavedlayer#2,\relax%
  \fi%
}
\newbox\pgf@layerboxsaved@main
\def\pgf@dosavelayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
    \setbox\pgf@layerboxsaved@main=\box\pgf@layerbox@main
  \else%
    \setbox\csname pgf@layerboxsaved@#1\endcsname=\box\csname pgf@layerbox@#1\endcsname%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dosavelayer#2,\relax%
  \fi%
}


\endinput

